Run for Cover: Dominating Set via Mobile Agents

Research involving computing with mobile agents is a fast-growing field, given the advancement of technology in automated systems, e.g., robots, drones, self-driving cars, etc. Therefore, it is pressing to focus on solving classical network problems using mobile agents. In this paper, we study one such problem -- finding small dominating sets of a graph $G$ using mobile agents. Dominating set is interesting in the field of mobile agents as it opens up a way for solving various robotic problems, e.g., guarding, covering, facility location, transport routing, etc. In this paper, we first present two algorithms for computing a {\em minimal dominating set}: (i) an $O(m)$ time algorithm if the robots start from a single node (i.e., gathered initially), (ii) an $O(\ell\Delta\log(\lambda)+n\ell+m)$ time algorithm, if the robots start from multiple nodes (i.e., positioned arbitrarily), where $m$ is the number of edges and $\Delta$ is the maximum degree of $G$, $\ell$ is the number of clusters of the robot initially and $\lambda$ is the maximum ID-length of the robots. Then we present a $\ln (\Delta)$ approximation algorithm for the {\em minimum} dominating set which takes $O(n\Delta\log (\lambda))$ rounds.

==> cds_rooted.tex <==
% \section{Connected Dominating Set using Mobile Robots (Rooted Initial Configuration)}
% A connected dominating set (CDS) of a graph is a dominating set such that the sub-graph induced by its vertices is connected. CDSs are helpful in the computation of routing for mobile ad hoc networks. In this application, a small connected dominating set is used as a backbone for communications, and nodes that are not in this set communicate by passing messages through neighbours that are in the set.

% In this section, we work out an algorithm that produces a CDS for an $n-node$ graph $G$ using mobile robots. Similar to our previous setting, $G$ is anonymous, memoryless, simple and connected. Such a setting is practically important since the nodes may choose not to disclose any information to the robots, due to security concerns. Therefore, the algorithm relies on mobile robots to store information and execute the algorithm; which sets this problem apart from classical graph algorithms. 

% In this problem, the robots start from a special node called the $root$. The robots use a DFS-based algorithm as described in Section~\ref{DFS} to reach a dispersed configuration where there is exactly one robot at each node. All the robots at this stage are coloured \textit{white}. To find the CDS, the robots need to associate themselves with a particular level (height) with respect to the root. For this, the robots use a variable $r_1.height$, initially assigned $null$. %Also, the robots receive new pointer information for $parent$ and $child$, which we incorporate using the variables $r_i.bfsparent$ and $r_i.bfschild$%. 
% %After the execution of the dispersion algorithm, a sub-protocol assigns the pointers on the robots ($r_i.bfsparent$ and $r_i.bfschild$) such that the DFS induced by the robots during dispersion now resents a BFS.% 
% After the end of the protocol, each robot receives a height (level) value. We call this protocol $assign\_height$, which we now explain below.

% The protocol $assign\_height$ runs phases, with each phase running for $\Delta$ rounds. Let us assume dispersion takes $T_{disperse}$ rounds to execute. After $T_{disperse}$ rounds, the minimum ID robot $r_1$, situated at the root sets its height as $0$ i.e, $r_1.height=0$. It then visits each neighbouring node and then activates and instructs each robot to set their $height\leftarrow r_1.height+1$. If the same robot receives multiple instructions (possibly, at some later stage of the protocol) for $height$ up-gradation, it ignores it. On the other hand, if a robot receives instruction from multiple robots, it obeys the instruction of the robot that has the least ID. Once the height for a robot has been set from $null$, it does not change during the algorithm. Now, after the end of the first phase, robots that are activated by $r_1$ scan each of their neighbours in parallel and consequently, instruct each of them to set their $height\leftarrow r_2.height+1$. As mentioned earlier, the robots that had their height set previously ignore any new instruction for $height$ change. 
% %Also, whenever a new robot $r_k$ finally receives a $height$ value from robot $r_p$, it notes the port through which $r_p$ exits and sets the same port as its $r_i.bfsparent$ pointer.In the next phase, when $r_i$ visits its neighbours, it can assign a height to some of the robots that initially had their $height$ set to $null.%
% We continue in a similar fashion until the end of the $n$ phases, after which every robot is guaranteed to have a unique height assigned to it. 

% After the height of each robot has been assigned, the algorithm proceeds to find the CDS for $G$. This part of the algorithm also runs in phases, where, each phase consists of $\Delta$ rounds. Initially, the $root$ robot $r_1$ colours itself \textit{black} and the phases begin. Now, in the first phase, the robots with $height=1$ scan their neighbourhood to check if there are any \textit{black} robots. If they find one (which is the case for all robots having $height=1$), the robots colour themselves \textit{grey}. Let's assume that, during the execution of the $i^{th}$ phase, $r_k$ is one such robot with $height=i$ scanning its neighbourhood. $r_k$ scans and checks if there are any \textit{black} robots in its neighbourhood. If $r_k$ doesn't find any \textit{black} robot, it colours itself \textit{grey} (contrary to previous cases, where a robot colours itself \textit{black}, upon finding that there are no black robots in the neighbourhood). $r_k$ then moves to its parent node and instructs the settled robot at the node to change its colour from \textit{grey} to \textit{black} and returns to its original node. Continuing in a similar fashion for $n$ rounds, each of the $n$ robots either receives a \textit{black} or a \textit{grey} colour. The nodes consisting of \textit{black} nodes form the CDS for graph $G$. We denote the set of nodes with black vertices as $D_{con}$.

% \subsection{Analysis}
% \begin{lemma}\label{lem:connected}
% $D_{con}\subset V$ represent a dominating set for $G$.
% \end{lemma}
% \begin{proof}
% For the contradiction, let us assume $D_{con}$ is not a dominating set for $G$. Therefore, there exists at least one node $x\in G\setminus D_{con}$ such that every neighbourhood of $x$ has a grey or a white robot. Now, there cannot be any white robot after the end of the algorithm, since every robot has a non-$null$ $height$ value and therefore must exhaustively receive a colour which is either \textit{grey} or \textit{black}. On the other hand, all the neighbourhoods of $x$ can not be grey, if so, the algorithm would re-colour of the parent of $x$ as \textit{black}. Therefore, any node of $G$ is either in $D_{con}$ or has a neighbouring node in $D_{con}$, making it a dominating set for $G$. 

% \end{proof}

% \begin{lemma}\label{lem:ds}
% $D_{con}\subset V$ is connected with respect to the graph $G$.
% \end{lemma}
% \begin{proof}
% Let us consider an arbitrary node $x\in D_{con}$. At some point of time, during the execution of the algorithm~\ref{alg: rooted_cds}, $x$ must have had all \textit{grey} neighbours. Then, it re-coloured its parent node (say $y$) to \textit{black}  from \textit{grey} according to the algorithm. Since $y$ was \textit{grey} earlier, it should have had a \textit{black} node $z$ as its parent. On the other side of the time, since $x$ eventually has become a member of $D_{con}$, one of its children must have coloured it \textit{black} at some later stage. Now, we see that the nodes $z-y-x$ that represent an arbitrary part of the set $D_{con}$ are connected. Therefore, in a similar fashion, we can argue that all the nodes in $D_{con}$ must be connected. 

% \end{proof}
% Combining Lemma~\ref{lem:ds} and Lemma~\ref{lem:connected}, we get the following
% \begin{lemma}
% The set $D_{con}\subset V$ represents a connected dominating set (CDS) for the graph $G$.
% \end{lemma}

% \begin{lemma}
% Algorithm~\ref{alg: rooted_cds} takes $O(n\Delta)$ rounds to complete.
% \end{lemma}
% \begin{proof}
% We first disperse the robot from a $rooted$ configuration which takes $O(m)$ rounds. For the protocol, $assign\_height$, $O(n\Delta)$ rounds are required, since there are $n$ phases each running for $\Delta$ rounds. Similarly, the last part of the algorithm that computes the CDS takes $O(n\Delta)$ rounds, since the same also runs in $n-1$ phases each requiring $\Delta$ rounds. Using the degree-sum formula, that gives  $n\Delta >m$, we can conclude that the Algorithm~\ref{alg: rooted_cds} takes $O(n\Delta)$ rounds to execute. 
% \end{proof}
% \begin{algorithm}[ht!]
%     \caption{\sc Rooted-Connected-Dominating-Set}
%     \begin{algorithmic}[1]
%     \Require{An anonymous network $G$ of $n$ nodes with $n$ mobile robots docked at node $R$}
%     \Ensure{Each individual robot identifies if it is a part dominating set $D$ of $G$}
%     \Statex
%     \State The set of $n$ robots $\mathcal{R}=\{r_1,r_2,\dots,r_n\}$ start at node $R$. Each robot $r_i$ maintains the following list of variables: $\langle r_i.id, r_i.parent, r_i.child, r_i.state, r_i.colour\rangle$. $r_i.colour$  is initially set to \textit{white}, $r_i.parent$, $r_i.child$ to $null$ and $r_i.state$ to \textit{forward}.  
%     \State The smallest ID robot $r_1$ at $R$ colours itself as \textit{black} and settles at R. The remaining unsettled robots move to a neighbouring port following the DFS Traversal Protocol~\ref{DFS}
%     \While{there is at least one \textit{white} robot}
%         \State The smallest ID robot $r_i$ among the group of unsettled robots settles at the new node. $r_i$ visits each of its neighbourhoods.
%         \If{at least one the neighbouring node has a \textit{black} robot}
%             \State colours itself as \textit{grey}
%         \Else 
%             \State colours itself as \textit{black}
%         \EndIf
%         \State The remaining unsettled robots exit via the appropriate port as per the DFS Protocol~\ref{DFS} and continue the DFS unless the robots find a new empty node.
%     \EndWhile
    

%     \State The nodes where each \textit{black}-coloured robot is stationed form the dominating set $D$ of $G$.
%     \end{algorithmic}
% \end{algorithm}\label{alg: rooted_cds}


\endinput

==> ds_arbitrary.tex <==
\section{Minimal Dominating Set for an Arbitrary Initial Configuration}\label{sec:arbitrary-config} 
In this case, the $n$ robots $\{r_1,r_2,\dots,r_n\}$ start as $\ell<n$ clusters, placed arbitrarily at $\ell$ different nodes of $G$. Once again, our algorithm for constructing dominating sets is inspired by the DFS procedure for dispersion~\cite{KS21}. 
% Briefly, each cluster (robots) independently computes its DFS in parallel and the corresponding dominating set with respect to the sub-graph it explores. To achieve this, each cluster (robots) begins in a similar procedure as in the rooted case and continues unless two or more DFSs meet. The meeting of two DFSs and the calculation of the dominating set thereafter is governed by several factors which are explained in the following subsection. 
% However, whenever two different DFS meet at a node, the smaller DFS (one that has a lesser number of robots settled) \anis{how do they know the number of settled robots?} gets subsumed by the larger one. After the subsumption, the settled robots from the smaller DFS get collected to the "head" of the larger one which then continues the DFS and builds on the dominating set.

% \anis{we should remove the questions para below...}
% While the procedure is simple, there are some complications that must be worked out. Such as:
% \begin{enumerate}
%     \item How do we identify the smaller DFS?
%     \item What if there are transitive chains of DFSs that are trying to subsume one another?   
%     \item What if a new DFS meets a DFS that is already executing some procedures (like subsuming/ getting subsumed)
%      \item How are the colours of the robots decided, when two different DFS meet?
%      \item Does the property of the local minimality in dominating sets transfer to the global one for $G$?
%    % \item How the dominating set, which is calculated locally by each cluster,  calculated for $G$?
% \end{enumerate}
% Through our algorithm, we sort out each of these complications to determine a dominating set for $G$with the last two questions being specific to creating dominating sets. 
We first provide a simple algorithm for finding a dominating set for $G$ that does not require the knowledge of $n,m$ or $\Delta$ apriori. Our initial approach, although simple, does not guarantee a minimal dominating set for $G$. In the worst case, it produces a dominating set of size as bad as $n$. In consequent subsections, we develop a new approach that guarantees a dominating set for $G$ which is globally minimal.  

\subsection{A Simple $O(m+n\Delta)$ Algorithm For Creating Dominating Set}
This algorithm is based on the \textit{dispersion} of mobile robots adapted from the procedure described by the authors in~\cite{KS21}. We adapt their dispersion procedure to create a protocol that also computes the dominating set. Crucially, the paper addresses the first three questions brought up in the previous section. In this section, we will first describe the dispersion algorithm, then we will show how with a few extra steps, we can, as in the rooted case, produce a dominating set algorithm for mobile robots. However, unlike the rooted case, this does not produce a minimal dominating set. In the later subsections, we show how, with the addition electing of a global leader, we can produce a minimal dominating set for $G$.  
\sumathi{\\\\If space is minimal, this can be moved to the appendix.}
\subsubsection{Step 1: Dispersing the Mobile Robots from an Arbitrary Initial Configuration: } 

We give a high-level idea of the dispersion algorithm used in~\cite{KS21}. The robots, along with the variables used in the rooted case, need two extra variables: $r_i.treelabel$ and $r_i.rank$. See~\ref{prelims} for details on the variables. 

%\sumathi{add a reference to the rooted section}   

%\sumathi{treelabel might be a better name than tree level as tree level usually indicates a level in the tree.}

\begin{enumerate}
    \item $r_i.treelabel$ - It is the ID of the minimum-ID robot in a particular cluster. It helps to differentiate between various DFSs.
    \item $r_i.rank$ - The first settled robot in a cluster has a rank $1$. Each successive robot that settles after it increases the $rank$ value by $1$.
\end{enumerate}
We identify a DFS as DFS $i$ if it has been induced by a cluster with $treelabel$ $i$. Each DFS with a distinct $treelabel$ originates from its initial cluster node, which we call the $root$. The $head$ of a DFS is the node which contains the robot with the highest $rank$. A robot can reach the $head$ of a DFS $i$ using $child$ pointers and the $root$ through $parent$ pointers. We say that a DFS $i$ meets DFS $j$ if the robots from DFS $i$ arrive at a node (called $junction$ $node$) where a robot from DFS $j$ already resides. When DFS $i$ meets DFS $j$, we say $head(i)$ is $blocked$.

When a DFS $i$ meets DFS $j$, the first task is to compare the sizes of the two DFSs, which is the number of settled robots in each DFS. For this, the unsettled of robots DFS $i$ at $head(i)$ traverse from the junction node to $head(j)$, reading the $rank$ of each robot on its way. If it finds a robot with a higher rank than its own size, then $d_i<d_j$ (here $d_i,d_j$ are the sizes DFS $i,j$ respectively). Otherwise, if it is able to reach $head(j)$ with encounter a robot with a higher rank than $d_i$, then $d_i>d_j$. The comparison can be performed in $O(\min(d_i,d_j))$.

After the sizes of the two DFS has been determined, the smaller DFS collapses by having all its robot collected at the $head$ of the larger DFS; which then continues the DFS as usual from the $head$. But, such collapses cannot occur immediately as the smaller DFS may have sent its own exploratory robots to another DFS it has just met. Also, due to concurrent actions happening in different parts of $G$ a DFS $j$ may be met by different other DFSs, and DFS $j$ may in turn meet other DFSs concurrently. There could be transitive chains of such meetings happening at the same time. When two DFSs meet, the algorithm determines its next course of action based on the findings of the exploratory robots, which explores the meeting DFS from the $juction$ $node$. There can be four possibilities: (i) the robots find a settled robot in the meeting DFS with a higher rank (ii) the robots reach the head of the meeting DFS without finding a robot with rank using its own DFS
(iii) robots learn that the meeting DFS is collapsing (or)
(iv) it meets with another exploratory robot, from a different DFS. Based on a particular case, the algorithm uses a proper ``locking" mechanism and may choose to execute among the following sub-protocols:
\begin{enumerate}
    \item $Collapse\_Into\_Parent(i)$ - This sub-protocol is invoked if a DFS $i$ meets another DFS of larger size and $head(i)$ is not locked. After the protocol is executed, the robots of the DFS $i$ collapse and gets collected at the $head$ of the larger DFS it has met. 
    \item $Collapse\_Into\_Child(i,j)$ - This sub-protocol is invoked if DFS $i$ meets another DFS $j$ of smaller size or if even if $i$ of larger size but its $head$, $head(i)$ has been locked by $j$. After the protocol is executed, the robots of the DFS $i$ collapse and gets collected at the $head$ of DFS $i$. 
    \item $Parent\_Is\_Collapsing$ - This is executed if the exploring robots of DFS $i$ find that the meeting DFS is collapsing or learn that the meeting DFS is locked and will be collapsing. This sub-protocol ensures that all the robots belonging to DFS $i$ also collapse with the DFS $j$ it has met, which itself is also collapsing if $d_j>d_i$. Otherwise, it waits until $j$'s collapse reaches $head(i)$ and then consumes all robots now accumulated at $head(i)$.
\end{enumerate}
A detailed account of the working of the dispersion algorithm can be found in~\cite{KS21}.
\subsubsection{Step 2: Finding a Dominating Set}
We now describe our algorithm for finding the dominating set. The robots from the $\ell$ clusters start their own DFS in parallel. As with the ``rooted'' case (Sec. ~\ref{sec:rooted-config}), the first robot, which has the lowest ID among its cluster, settles and marks itself as \textit{black}. As mentioned, the robots also have a variable called $treelabel$ which helps to differentiate itself from the robots from another cluster. The others, except for the settled robot exit via a suitable port according to the DFS Protocol~\ref{DFS}. The next robot (the one with the next lowest ID) now settles at the new node. It visits each neighbour and checks if there is a \textit{black} robot with the same $treelabel$ as itself. If yes, it settles and marks itself \textit{grey} otherwise, it marks itself as \textit{black}. Note that while exploring the neighbours, a robot from DFS $i$ could find settled robots from a different DFS $j$, however, it ignores all robots except the ones belonging to its own DFS (note, this is because the placement of robots is not permanent and is dependent on the other DFSs running parallel). The algorithm continues as usual before DFSs start meeting one another. 

When a DFS $i$ meets another DFS $j$, the dispersion algorithm of~\cite{KS21} takes over. The shorter DFS gets subsumed into the larger one and all the robots move to the $head$ of the larger DFS. Once the robots in shorter DFS are informed about the ``subsumption '', all the robots change their colour to \textit{white}. Once, the DFS gets to resume from the $head$ (with now, a large number of unsettled robots), the colouring continues as usual. Similarly, for all the other cases, whenever a collapse of robots occurs, all the collapsing robots reset their $colour$ to \textit{white}. The robots get eventually collected at the $head$ of some DFS, after which the DFS continues exploration in a similar fashion to the rooted case. At the end of the algorithm, each node has a settled robot that is either coloured \textit{grey} or \textit{black}. The nodes that have a \textit{black} robot at the end of the algorithm, mark the dominating set for the graph $G$.




\subsubsection{Analysis}
\sumathi{check notation for $D$}
\begin{lemma}
Algorithm~\ref{alg: arbitrary_ds_each_robot_basic} produces a dominating set $D \subseteq V$ for graph $G$ identified by the set of \textit{black} coloured robots. 
\end{lemma}
\sumathi{this proof is not clear to me\\}
\prabhat{revised\\}
\begin{proof} 
Let us assume that Algorithm~\ref{alg: arbitrary_ds_each_robot_basic} leaves $c<\ell$ independent DFSs with $c$ distinct $treelabel$s at the end of the algorithm, as some DFSs could meet each other and get absorbed into one, during the process. Now we consider the $c$ DFS sub-trees $T_1,T_2,T_3,\dots,T_c$ induced by these $c$ DFSs. With a similar argument, as used for the rooted case, it can be shown that the set of nodes with \textit{black} robots in $T_i$ gives a local dominating set for the sub-graph $G_i\subset G$ induced by the nodes in $T_i$. Therefore every node of $G_i$ is covered by some \textit{black} robot. Since there are exactly $n$ robots placed at $n$ node of $G$ and every node is a member of one of the $c$ sub-trees, therefore for any node $v\in G$, $v$ must be a member of exactly one of the sub-trees $T_1,T_2,T_3,\dots,T_c$. Therefore, either $v$ must be \textit{black} or \textit{grey}. Since $v$ is arbitrary, every node of $G$ is covered. Hence, the nodes with \textit{black} robots form a dominating set $D$ for $G$.  

\end{proof}

\begin{remark}
The set $D\subset V$ may not be a maximal independent set for $G$, since there could be two adjacent \textit{black} robots (each belonging to a different DFS). 
\end{remark}

% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
% {\caption{A test figure with its caption side by side}\label{fig:test}}
% {\includegraphics[scale=0.38]{figures/non_minimal_arbitrary.png}}
% \end{figure}


\begin{figure}[!ht]
  \centering
    \includegraphics[scale=0.38]{figures/non_minimal_arbitrary.png}
  \caption{Illustration of Algorithm~\ref{alg: arbitrary_ds_each_robot_basic} failing to produce a minimal dominating set. DFS $i$, beginning at node $C$ goes through nodes A,B,E,D,G,I and J and colours the robots on them accordingly (blue coloured edges). As DFS $i$ colours the robot at C as \textit{black}, at the same time, the single robot DFS $p$ colours the robot at F as \textit{black}, which is redundant in respect of the minimality of the dominating set for graph $G$. A more trivial example one may think about is when the robots begin in a dispersed position and there are $n$ independent DFSs and every robot becomes \textit{black}. \anis{try to place the caption to the side of the figure, not below. This will save some space.}\prabhat{I have tried a code for this. Not working. I am on it. }}\label{fig:non_minimal_DS}
  \end{figure}

\begin{remark}
Algorithm~\ref{alg: arbitrary_ds_each_robot_basic} requires \textbf{no} knowledge of $m,n$ or $\Delta$.
\end{remark}

\begin{lemma}
    Algorithm~\ref{alg: arbitrary_ds_each_robot_basic} takes $O(m+n\Delta)$ rounds to execute.
\end{lemma}

\sumathi{this part is unclear. perhaps reference how much time KS21 takes to collapse down and include that.\\}
\prabhat{Revised. }
\begin{proof}
    The algorithm can be split into two parts - a dispersion of the mobile robots that were initially clustered arbitrarily and finding a local dominating set for each independently running DFS. To simplify the time complexity analysis, we calculate the dispersion time and time for dominating set identification separately since the steps for dispersion are mutually exclusive to the steps required for finding the dominating set. Now, due to \cite{KS21}, dispersion along with all its included sub-protocols takes $O(m)$ rounds. 
    
    If the DFSs never meet, the dominating set can be discovered in $O(m+n\Delta)$ rounds since the time only depends on the largest cluster with the maximum number the robots. The largest cluster may take $O(m)$ rounds to disperse and additional $O(n\Delta)$ rounds to find the dominating set (as shown in the rooted case \ref{alg: rooted_ds}). On the other hand, let's assume that some of the DFSs meet during the algorithm and let DFS $p$ be the largest DFS among all the meeting DFSs (denoted by $master$ $node$ in \cite{KS21}). Now, since $p$ is the largest DFS, all other DFS that meets $p$ ultimately get collected at the head of DFS $p$. The DFSs that collapse and meet $p$ may have partly identified its local dominating set, however, such steps occur in parallel with DFSs $p$ and hence do not contribute to the time complexity. Therefore, the time taken by the largest DFS $p$ dominates the time complexity. At worst, $p$ may have to subsume all other DFSs one by one serially and consume $O(n\Delta)$ rounds before the algorithm ends. 
\end{proof}

\begin{algorithm}[ht!]
    \caption{\sc Arbitrary-Dominating-Set}
    \begin{algorithmic}[1]
    \Require{A robot cluster consisting of $b<n$ mobile robots docked at node $x\in G$ }
    \Ensure{Each individual robot identifies if it is a part dominating set $D$ of $G$}
    \Statex
    \State The set of $b<n$ robots start at node $x$. Each robot $r_i$ maintains the following list of variables: $\langle r_i.id, r_i.parent, r_i.child, r_i.state,r_i.treelabel,r_i.rank, r_i.colour\rangle$. $r_i.colour$  is initially set to \textit{white}, $r_i.parent$, $r_i.child$ to $null$ and $r_i.state$ to \textit{forward}.  
    \State The smallest ID robot $r$ from the cluster colours itself as \textit{black} and settles at $x$. The remaining unsettled robots move to a neighbouring port following the DFS Traversal Protocol~\ref{DFS}
    \While{there is at least one \textit{white} robot in the cluster}
        \State The smallest ID robot $r_i$ among the group of unsettled robots settles at the new node. $r_i$ visits each of its neighbourhoods.
        \If{at least one the neighbouring node has a \textit{black} robot with same $treelabel$ as itself}
            \State $r_i$ colours itself as \textit{grey}
        \Else 
            \State $r_i$ colours itself as \textit{black}
        \EndIf
        \State The remaining unsettled robots exit via the appropriate port as per the DFS Protocol~\ref{DFS} and continue the DFS unless the robots find a new empty node or it meets another $DFS$.
        \If{$r_i$ meets a settled robot from a different $treelabel$}
            \State follow the appropriate procedure for subsumption  from Algorithm~\cite{KS21}
            \If{$r_i$ is collapsing/being subsumed}
                \State $r_i$ colours itself as \textit{white}
                \State break;
            \EndIf
            \State Wait for the sub-protocols to complete, continue on completion
        \Else 
            \State continue
        \EndIf
    \EndWhile
    \end{algorithmic}
\end{algorithm}\label{alg: arbitrary_ds_each_robot_basic}

\subsection{Creating a Minimal Dominating Set}\label{mds_arbitrary}
Although the procedure described in the previous section yields a dominating set for graph $G$, it does not guarantee that the dominating set is minimal. However, we show that we can create a minimal dominating set if we trade off on time. We now give an algorithm below that invests more on time but guarantees a minimal dominating set. The algorithm takes $O(\ell\Delta\log(\lambda)+n\ell+n\Delta)$ rounds (where $\lambda$ is the number of bits required to represent a robot's ID), compared to the previous algorithm which takes $O(m+n\Delta)$ rounds. This algorithm also requires the knowledge of $n,\Delta,\ell$ and $\lambda$ (parameters are defined in Section~\ref{prelims}).

% The figure \sumathi{what figure?} given below describes one such situation in which our previous Algorithm~\ref{alg: arbitrary_ds_each_robot_basic} may fail to give a minimal dominating set for the arbitrary starting configuration. 

One of the key reasons that our previous algorithm does not give us a minimal set is the absence of communication and synchronisation among the parallelly running DFSs. This leads to more number of robots receiving \textit{black} colour than required. For example, a cluster with a single robot colours itself black according to the algorithm, which may be redundant, if that particular node is already covered by another black robot. This demands an alteration in the existing algorithm. In this algorithm, we first disperse the mobile robots to each node, then choose a global leader, which orchestrates the creation of a minimal dominating set using the same procedures as in the rooted case.  

The robots first perform dispersion using the method described in Kshemkalyani\cite{KS21}. Robots from the $\ell$ clusters independently build on the DFS as they disperse the robots one by one. When two DFSs meet, the shorter DFS gets subsumed by the larger one. Let us assume, after the end of the algorithm, there are $c\leq \ell$ independent DFSs that never met. Note that each DFS is identified by a variable $treelabel$, the ID of the smallest robot in the cluster. When two DFS meet, the subsumed robots have their $treelabel$ changed according to DFS that is subsuming it. Therefore, the final $c$ DFSs that remain have a distinct $treelabel$ which is the same across all the robots in that DFS, even though some robots of them may have joined later. After the robots have been dispersed, we proceed to select a global leader without which, it is difficult to synchronise the activities executed in each DFS. Each among the $c$ DFSs locally knows the lowest ID robot in its DFS, however, the global minimum is unknown since there is no scope of communication between robots of different DFSs. To get a leader robot, we proceed as follows. 

% \noindent\textbf{Brief Summary:} \sumathi{Explain what is meant by upcast and downcast} 
Let $P$ be a protocol that allows a robot to scan its neighbourhood within $T$ rounds (details of $P$ and $T$ are given below in Section~\ref{prelims}). When a robot meets another robot from a different ID, they share their $treelabel$s with one another. When a robot receives a lower $treelabel$ value, it updates its own $treelabel$ to the lower value. After $P$ has been executed (realised by the end of $T$ rounds), %each robot in the DFS $i$, except the one designated as a root $root_i$, follows $parent$ pointers to reach $root_i$ to submit the recently updated $treelabel$ value. $root_i$ now selects the minimum among all the received $treelabel$ values and shares it with the other robots, now gathered at $root_i$. All robots now leave $root_i$ with the updated $treelabel$ value to their original%
each robot, starting from the leaf nodes in a DFS (say DFS $i$) now sends its newly updated $treelabel$ value to the root of DFS ($root_i$) via its $parent$ pointers. The root of the DFS $i$, $root_i$, waits for $O(n)$ rounds as it receives different values of $treelabel$ continuously from its leaf nodes (\textit{up-casting}). The $root_i$ now compares the minimum $treelabel$ values received from its children with its own $treelabel$ and decides on the minimum $treelabel$. It then sends it along through its children into each and every node of its in the DFS (\textit{down-casting}). All the robots in DFS $i$ are now updated with the lowest $treelabel$ value. This marks the end of a phase. After the end of $\ell$ (although $c$ is sufficient, its value is unknown) such phases, it is guaranteed that each of the $n$ robots in $G$ now has a consistent $treelabel$ value. The final $treelabel$ value is the minimum among the $c$ DFSs, however, it may not represent the minimum $ID$ robot, as it may be consumed by a larger DFS during the dispersion process happening earlier. After the end of the protocol, the robot that has the globally decided minimum $treelabel$ continues the algorithm. We assume the leader robot with the minimum $treelabel$ value as $r^\star$.

% After the end of the protocol, each robot receives a height (level) value. We call this protocol $assign\_height$, which we now explain below.

% The protocol $assign\_height$ runs phases, with each phase running for $\Delta$ rounds. The leader robot $r^\star$ sets its height as $0$ i.e., $r^\star.height=0$. It then visits each neighbouring node and then activates and instructs each robot to set their $height\leftarrow r^\star.height+1$. If the same robot receives multiple instructions (possibly, at some later stage of the protocol) for $height$ up-gradation, it ignores it. On the other hand, if a robot receives instruction from multiple robots, it obeys the instruction of the robot that has the least ID. Once the height for a robot has been set from $null$, it does not change during the algorithm. Now, after the end of the first phase, robots that are activated by $r^\star$ scan each of their neighbours in parallel and consequently, instruct each of them to set their height which is one more than its parent's height. In the meanwhile, $r^\star$, returns to its original node. As mentioned earlier, the robots that had their height set previously ignore any new instruction for $height$ change. 
% %Also, whenever a new robot $r_k$ finally receives a $height$ value from robot $r_p$, it notes the port through which $r_p$ exits and sets the same port as its $r_i.bfsparent$ pointer.In the next phase, when $r_i$ visits its neighbours, it can assign a height to some of the robots that initially had their $height$ set to $null.%
% We continue in a similar fashion until the end of the $n$ phases, after which every robot is guaranteed to have a unique height assigned to it. Also, by the end of the procedure, each robot is now at its original node as it was, before the start of the algorithm. 

% After the height of each robot has been assigned, the algorithm proceeds to find the dominating set for $G$. This part of the algorithm also runs in phases, where, each phase consists of $\Delta$ rounds. Initially, $r^\star$ colours itself \textit{black} and the phases begin. Now, in the first phase, the robots with $height=1$ scan their neighbourhood to check if there are any \textit{black} robots. If they find one (which is the case for all robots having $height=1$), the robots colour themselves \textit{grey}. Let's assume that, during the execution of the $i^{th}$ phase, $r_k$ is one such robot with $height=i$ scanning its neighbourhood. $r_k$ scans and checks if there are any \textit{black} robots in its neighbourhood. If $r_k$ doesn't find any \textit{black} robot, it colours itself \textit{black} Continuing in a similar fashion for $n$ rounds, each of the $n$ robots either receives a \textit{black} or a \textit{grey} colour. The nodes consisting of \textit{black} nodes form the dominating set for graph $G$. We denote the set of nodes with black vertices as $D$.

With $r^\star$ as a leader, it first creates a new DFS of the graph $G$ with the node containing $r^\star$ as the $root$ node. Since the robots are dispersed across each and every node of $G$, the nodes of $G$ are now distinguishable owing to the distinct IDs of the mobile robots in the nodes. $r^\star$  starts from the root and rewrites the $parent$ and $child$ pointers of each robot as its traverses across the whole graph $G$ in a depth-first manner. Moving to an empty node implies that $r^\star$ has arrived at the $root$. In such cases, $r^\star$ modifies its own variables accordingly. The other details regarding the DFS can be found in section~\ref{DFS}. After the end of this process, which takes an additional $O(m)$ rounds, the newly assigned pointers of the robots now represent a DFS of $G$ with $r^\star$ (node) as the root.

Initially, all the robots are coloured \textit{white} by default. The identification of the dominating set takes place in similar lines as with the rooted case described in the previous section~\ref{alg: rooted_ds}. The algorithm begins with $r^\star$ colouring itself black. $r^\star$ then moves the next node (say node $u$ resided by a robot $r_u$) following the newly created DFS. Upon the arrival of $r^\star$ at $u$, $r_u$ scans each of its neighbours to check if there is a black robot. If there are no black robots, $r_u$ colours itself as \textit{black} otherwise if there is at least one black robot in the neighbourhood of $u$, $r_u$ colours itself \textit{grey}. After $r_u$ has changed its colour from \textit{white}, it informs $r^\star$ as $r^\star$ now moves to the next node following the DFS. The process continues similarly with each new node taking $O(\Delta)$ rounds its scan its neighbour and colour itself accordingly. The algorithm terminates as soon as $r^\star$ completes the DFS of $G$.  

% \subsubsection{Details of the Procedure $P$ and Time $T$} \sumathi{Should we include this in the prelim section as we are using it twice?}
% Here we explain how the robots scan their neighbourhood. For this, the algorithm essentially exploits the bits representing the IDs of the robots. Let $\lambda$ denote the largest ID among all the $n$ robots. Therefore, the robots use a $\log \lambda$ bit field to store the IDs. $P$ runs in phases. Each phase has $\Delta$ rounds and there are a total of  $\log \lambda$ phases. Now, to find the neighbouring robots, a robot $r_i$ stationed at a node $u$ does the following.
% \begin{enumerate}\label{procedure1}
%     \item Checks the rightmost bit in its ID field. 
%     \item If the bit is $1$, $r_i$ goes to each of its neighbours one by one from $u$ following ascending order of the port numbers and back. Note that, from $u$, there are ports numbered from $0$ to $\delta_u-1$  each leading to a distinct neighbour of $u$.
%     \item If $r_i$ finds a robot $r_j$ (or other multiple robots) in its neighbour, each robot updates the $treelabel$ value with the minimum value among themselves, including $r_i$ itself.
%     \item Otherwise, if the bit id $0$, the robots sits at $u$ and waits for $\Delta$ rounds. 
%     \item In the next phase of $\Delta$ rounds, $r_i$ now checks its second bit from the right and repeats the same process as described in the previous steps.   
%     \item The process continues for $\log \lambda$ phases, ensuring every bit in the ID field has been scanned. If there are no more bits remaining in $r_i.ID$ and $\log\lambda$ rounds have not been completed (implying that $r_i$ has a smaller ID length than $\log\lambda$ bits), $r_i$ assumes the current bit as $0$ and stays back at its own node for the rest part of the algorithm. 
% \end{enumerate}
% Each execution of procedure $P$ takes $T=O(\Delta\log \lambda)$ rounds.


% \begin{algorithm}[ht!]
%     \caption{\sc Arbitrary-Minimal-Dominating-Set}
%     \begin{algorithmic}[1]
%     \Require{A robot cluster consisting of $b<n$ mobile robots docked at node $x\in G$ }
%     \Ensure{Each individual robot identifies if it is a part dominating set $D$ of $G$}
%     \Statex
%     \State The set of $b<n$ robots start at node $x$. Each robot $r_i$ maintains the following list of variables: $\langle r_i.id, r_i.parent, r_i.child, r_i.state,r_i.treelabel,r_i.rank, r_i.colour\rangle$. $r_i.colour$  is initially set to \textit{white}, $r_i.parent$, $r_i.child$ to $null$ and $r_i.state$ to \textit{forward}.  
%     \State The robots perform \textsc{dispersion} using the procedure described in Kshemkalyani \etal~\cite{KS21} 
%     \For{this}
%     \State Hello
%     \EndFor
%     \end{algorithmic}
% \end{algorithm}\label{alg: arbitrary_ds_each_robot}


% \begin{algorithm}[ht!]
%     \caption{\sc Procedure $P$}
%     \begin{algorithmic}[1]
%     \Require{A mobile robot $r_i$ with $\log\lambda$ bit ID field - $b_1b_2...b_{k}$; $k\leq\log\lambda$}
%     \Ensure{$r_i$ meets every other robot in its neighbourhood}
%     \Statex
%     \For{$\log\lambda$ rounds}
%         \State $r_i$ checks the current bit in its ID field starting from the rightmost bit $b_k$. 
%         \If{concerned bit is $1$}, 
%             \State $r_i$ gets a phase of $\Delta$ rounds where it goes to each of its neighbours one by one from $u$ (its station node) following ascending order of the port numbers and back. When it meets a new robot at its neighbour, the two update the 'minimum ID' information.
%         \Else {$r_i$ remains stationary at $u$ and waits for $\Delta$ rounds (phase to complete). If $r_i$ has a visitor, the robots update the 'minimum ID' information.}
%         \EndIf
%     \State After the completion of the ongoing phase of $\Delta$ rounds, the next left bit in the ID field of $r_i$ becomes the concerned bit. If there are no more bits remaining in $r_i.ID$ set the current bit as $0$ and stay at the same node. 
%     \EndFor
%     \end{algorithmic}
% \end{algorithm}\label{alg: procedure_P}

We conclude the section with its main theorem. 
\begin{theorem}
   
        Let $G$ be an $n$ node arbitrary, simple, connected graph with a maximum degree $\Delta$. Let $n$ mobile robots with distinct IDs in the range $[0,n^c]$, where $c$ is constant, be initially placed arbitrarily among the nodes of $G$. Then, a minimal dominating set for $G$ can be found in $OO(\ell\Delta\log(\lambda)+n\ell+n\Delta)$ rounds using Algorithm~\ref{mds_arbitrary} with $O(\log n)$ bits of memory per robot. Here, $\Delta$ is the maximum degree of a node in $G$ and $\lambda$ is the $ID$ length of the robot with the highest $ID$. 

     % (\sumathi{length or value, length implies number of bits}) of the robot with the highest $ID$. 
\end{theorem}
\begin{proof}
    Algorithm~\ref{mds_arbitrary} first disperses the robots, which takes $O(m)$ rounds. We then elect a global leader. There are $\ell$ clusters at most, and each cluster uses procedure $P$ to communicate with neighbouring clusters. In the worst case, to get the leader robot, $P$ must be executed $\ell$ times since the DFS induced by the $\ell$ clusters can be end-to-end. Once the leaf nodes receive a new communication from a different cluster, it needs $O(n)$ rounds to transmit it to the local root of the cluster. The leader robot then creates a DFS in $O(m)$ and then, the dominating set identification takes another $O(n\Delta)$ rounds. Therefore, algorithm~\ref{mds_arbitrary} has an execution time of $O(m)+O(\ell(\Delta\log\lambda+n))+O(n\Delta)$ rounds. 
    
    The memory requirement remains the same as in the rooted case except for some constant number of extra variables used here.
\end{proof}
\endinput

==> extra.tex <==
\section*{Appendix (Full paper attached)}\label{sec:appendix}

\endinput


==> literature.tex <==
% LLNCS DOCUMENT CLASS -- version 2.20 (10-Mar-2018)
% Springer Verlag LaTeX2e support for Lecture Notes in Computer Science
%
%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{llncs}[2018/03/10 v2.20
^^J LaTeX document class for Lecture Notes in Computer Science]
% Options
\let\if@envcntreset\iffalse
\DeclareOption{envcountreset}{\let\if@envcntreset\iftrue}
\DeclareOption{citeauthoryear}{\let\citeauthoryear=Y}
\DeclareOption{oribibl}{\let\oribibl=Y}
\let\if@custvec\iftrue
\DeclareOption{orivec}{\let\if@custvec\iffalse}
\let\if@envcntsame\iffalse
\DeclareOption{envcountsame}{\let\if@envcntsame\iftrue}
\let\if@envcntsect\iffalse
\DeclareOption{envcountsect}{\let\if@envcntsect\iftrue}
\let\if@runhead\iffalse
\DeclareOption{runningheads}{\let\if@runhead\iftrue}

\let\if@openright\iftrue
\let\if@openbib\iffalse
\DeclareOption{openbib}{\let\if@openbib\iftrue}

% languages
\let\switcht@@therlang\relax
\def\ds@deutsch{\def\switcht@@therlang{\switcht@deutsch}}
\def\ds@francais{\def\switcht@@therlang{\switcht@francais}}

\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}

\ProcessOptions

\LoadClass[twoside]{article}
\RequirePackage{multicol} % needed for the list of participants, index
\RequirePackage{aliascnt}

\setlength{\textwidth}{12.2cm}
\setlength{\textheight}{19.3cm}
\renewcommand\@pnumwidth{2em}
\renewcommand\@tocrmarg{3.5em}
%
\def\@dottedtocline#1#2#3#4#5{%
  \ifnum #1>\c@tocdepth \else
    \vskip \z@ \@plus.2\p@
    {\leftskip #2\relax \rightskip \@tocrmarg \advance\rightskip by 0pt plus 2cm
               \parfillskip -\rightskip \pretolerance=10000
     \parindent #2\relax\@afterindenttrue
     \interlinepenalty\@M
     \leavevmode
     \@tempdima #3\relax
     \advance\leftskip \@tempdima \null\nobreak\hskip -\leftskip
     {#4}\nobreak
     \leaders\hbox{$\m@th
        \mkern \@dotsep mu\hbox{.}\mkern \@dotsep
        mu$}\hfill
     \nobreak
     \hb@xt@\@pnumwidth{\hfil\normalfont \normalcolor #5}%
     \par}%
  \fi}
%
\def\switcht@albion{%
\def\abstractname{Abstract.}
\def\ackname{Acknowledgement.}
\def\andname{and}
\def\lastandname{\unskip, and}
\def\appendixname{Appendix}
\def\chaptername{Chapter}
\def\claimname{Claim}
\def\conjecturename{Conjecture}
\def\contentsname{Table of Contents}
\def\corollaryname{Corollary}
\def\definitionname{Definition}
\def\examplename{Example}
\def\exercisename{Exercise}
\def\figurename{Fig.}
\def\keywordname{{\bf Keywords:}}
\def\indexname{Index}
\def\lemmaname{Lemma}
\def\contriblistname{List of Contributors}
\def\listfigurename{List of Figures}
\def\listtablename{List of Tables}
\def\mailname{{\it Correspondence to\/}:}
\def\noteaddname{Note added in proof}
\def\notename{Note}
\def\partname{Part}
\def\problemname{Problem}
\def\proofname{Proof}
\def\propertyname{Property}
\def\propositionname{Proposition}
\def\questionname{Question}
\def\remarkname{Remark}
\def\seename{see}
\def\solutionname{Solution}
\def\subclassname{{\it Subject Classifications\/}:}
\def\tablename{Table}
\def\theoremname{Theorem}}
\switcht@albion
% Names of theorem like environments are already defined
% but must be translated if another language is chosen
%
% French section
\def\switcht@francais{%\typeout{On parle francais.}%
 \def\abstractname{R\'esum\'e.}%
 \def\ackname{Remerciements.}%
 \def\andname{et}%
 \def\lastandname{ et}%
 \def\appendixname{Appendice}
 \def\chaptername{Chapitre}%
 \def\claimname{Pr\'etention}%
 \def\conjecturename{Hypoth\`ese}%
 \def\contentsname{Table des mati\`eres}%
 \def\corollaryname{Corollaire}%
 \def\definitionname{D\'efinition}%
 \def\examplename{Exemple}%
 \def\exercisename{Exercice}%
 \def\figurename{Fig.}%
 \def\keywordname{{\bf Mots-cl\'e:}}
 \def\indexname{Index}
 \def\lemmaname{Lemme}%
 \def\contriblistname{Liste des contributeurs}
 \def\listfigurename{Liste des figures}%
 \def\listtablename{Liste des tables}%
 \def\mailname{{\it Correspondence to\/}:}
 \def\noteaddname{Note ajout\'ee \`a l'\'epreuve}%
 \def\notename{Remarque}%
 \def\partname{Partie}%
 \def\problemname{Probl\`eme}%
 \def\proofname{Preuve}%
 \def\propertyname{Caract\'eristique}%
%\def\propositionname{Proposition}%
 \def\questionname{Question}%
 \def\remarkname{Remarque}%
 \def\seename{voir}
 \def\solutionname{Solution}%
 \def\subclassname{{\it Subject Classifications\/}:}
 \def\tablename{Tableau}%
 \def\theoremname{Th\'eor\`eme}%
}
%
% German section
\def\switcht@deutsch{%\typeout{Man spricht deutsch.}%
 \def\abstractname{Zusammenfassung.}%
 \def\ackname{Danksagung.}%
 \def\andname{und}%
 \def\lastandname{ und}%
 \def\appendixname{Anhang}%
 \def\chaptername{Kapitel}%
 \def\claimname{Behauptung}%
 \def\conjecturename{Hypothese}%
 \def\contentsname{Inhaltsverzeichnis}%
 \def\corollaryname{Korollar}%
%\def\definitionname{Definition}%
 \def\examplename{Beispiel}%
 \def\exercisename{\"Ubung}%
 \def\figurename{Abb.}%
 \def\keywordname{{\bf Schl\"usselw\"orter:}}
 \def\indexname{Index}
%\def\lemmaname{Lemma}%
 \def\contriblistname{Mitarbeiter}
 \def\listfigurename{Abbildungsverzeichnis}%
 \def\listtablename{Tabellenverzeichnis}%
 \def\mailname{{\it Correspondence to\/}:}
 \def\noteaddname{Nachtrag}%
 \def\notename{Anmerkung}%
 \def\partname{Teil}%
%\def\problemname{Problem}%
 \def\proofname{Beweis}%
 \def\propertyname{Eigenschaft}%
%\def\propositionname{Proposition}%
 \def\questionname{Frage}%
 \def\remarkname{Anmerkung}%
 \def\seename{siehe}
 \def\solutionname{L\"osung}%
 \def\subclassname{{\it Subject Classifications\/}:}
 \def\tablename{Tabelle}%
%\def\theoremname{Theorem}%
}

% Ragged bottom for the actual page
\def\thisbottomragged{\def\@textbottom{\vskip\z@ plus.0001fil
\global\let\@textbottom\relax}}

\renewcommand\small{%
   \@setfontsize\small\@ixpt{11}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \parsep 0\p@ \@plus1\p@ \@minus\p@
               \topsep 8\p@ \@plus2\p@ \@minus4\p@
               \itemsep0\p@}%
   \belowdisplayskip \abovedisplayskip
}

\frenchspacing
\widowpenalty=10000
\clubpenalty=10000

\setlength\oddsidemargin   {63\p@}
\setlength\evensidemargin  {63\p@}
\setlength\marginparwidth  {90\p@}

\setlength\headsep   {16\p@}

\setlength\footnotesep{7.7\p@}
\setlength\textfloatsep{8mm\@plus 2\p@ \@minus 4\p@}
\setlength\intextsep   {8mm\@plus 2\p@ \@minus 2\p@}

\setcounter{secnumdepth}{2}

\newcounter {chapter}
\renewcommand\thechapter      {\@arabic\c@chapter}

\newif\if@mainmatter \@mainmattertrue
\newcommand\frontmatter{\cleardoublepage
            \@mainmatterfalse\pagenumbering{Roman}}
\newcommand\mainmatter{\cleardoublepage
       \@mainmattertrue\pagenumbering{arabic}}
\newcommand\backmatter{\if@openright\cleardoublepage\else\clearpage\fi
      \@mainmatterfalse}

\renewcommand\part{\cleardoublepage
                 \thispagestyle{empty}%
                 \if@twocolumn
                     \onecolumn
                     \@tempswatrue
                   \else
                     \@tempswafalse
                 \fi
                 \null\vfil
                 \secdef\@part\@spart}

\def\@part[#1]#2{%
    \ifnum \c@secnumdepth >-2\relax
      \refstepcounter{part}%
      \addcontentsline{toc}{part}{\thepart\hspace{1em}#1}%
    \else
      \addcontentsline{toc}{part}{#1}%
    \fi
    \markboth{}{}%
    {\centering
     \interlinepenalty \@M
     \normalfont
     \ifnum \c@secnumdepth >-2\relax
       \huge\bfseries \partname~\thepart
       \par
       \vskip 20\p@
     \fi
     \Huge \bfseries #2\par}%
    \@endpart}
\def\@spart#1{%
    {\centering
     \interlinepenalty \@M
     \normalfont
     \Huge \bfseries #1\par}%
    \@endpart}
\def\@endpart{\vfil\newpage
              \if@twoside
                \null
                \thispagestyle{empty}%
                \newpage
              \fi
              \if@tempswa
                \twocolumn
              \fi}

\newcommand\chapter{\clearpage
                    \thispagestyle{empty}%
                    \global\@topnum\z@
                    \@afterindentfalse
                    \secdef\@chapter\@schapter}
\def\@chapter[#1]#2{\ifnum \c@secnumdepth >\m@ne
                       \if@mainmatter
                         \refstepcounter{chapter}%
                         \typeout{\@chapapp\space\thechapter.}%
                         \addcontentsline{toc}{chapter}%
                                  {\protect\numberline{\thechapter}#1}%
                       \else
                         \addcontentsline{toc}{chapter}{#1}%
                       \fi
                    \else
                      \addcontentsline{toc}{chapter}{#1}%
                    \fi
                    \chaptermark{#1}%
                    \addtocontents{lof}{\protect\addvspace{10\p@}}%
                    \addtocontents{lot}{\protect\addvspace{10\p@}}%
                    \if@twocolumn
                      \@topnewpage[\@makechapterhead{#2}]%
                    \else
                      \@makechapterhead{#2}%
                      \@afterheading
                    \fi}
\def\@makechapterhead#1{%
% \vspace*{50\p@}%
  {\centering
    \ifnum \c@secnumdepth >\m@ne
      \if@mainmatter
        \large\bfseries \@chapapp{} \thechapter
        \par\nobreak
        \vskip 20\p@
      \fi
    \fi
    \interlinepenalty\@M
    \Large \bfseries #1\par\nobreak
    \vskip 40\p@
  }}
\def\@schapter#1{\if@twocolumn
                   \@topnewpage[\@makeschapterhead{#1}]%
                 \else
                   \@makeschapterhead{#1}%
                   \@afterheading
                 \fi}
\def\@makeschapterhead#1{%
% \vspace*{50\p@}%
  {\centering
    \normalfont
    \interlinepenalty\@M
    \Large \bfseries  #1\par\nobreak
    \vskip 40\p@
  }}

\renewcommand\section{\@startsection{section}{1}{\z@}%
                       {-18\p@ \@plus -4\p@ \@minus -4\p@}%
                       {12\p@ \@plus 4\p@ \@minus 4\p@}%
                       {\normalfont\large\bfseries\boldmath
                        \rightskip=\z@ \@plus 8em\pretolerance=10000 }}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                       {-18\p@ \@plus -4\p@ \@minus -4\p@}%
                       {8\p@ \@plus 4\p@ \@minus 4\p@}%
                       {\normalfont\normalsize\bfseries\boldmath
                        \rightskip=\z@ \@plus 8em\pretolerance=10000 }}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                       {-18\p@ \@plus -4\p@ \@minus -4\p@}%
                       {-0.5em \@plus -0.22em \@minus -0.1em}%
                       {\normalfont\normalsize\bfseries\boldmath}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                       {-12\p@ \@plus -4\p@ \@minus -4\p@}%
                       {-0.5em \@plus -0.22em \@minus -0.1em}%
                       {\normalfont\normalsize\itshape}}
\renewcommand\subparagraph[1]{\typeout{LLNCS warning: You should not use
                  \string\subparagraph\space with this class}\vskip0.5cm
You should not use \verb|\subparagraph| with this class.\vskip0.5cm}

\DeclareMathSymbol{\Gamma}{\mathalpha}{letters}{"00}
\DeclareMathSymbol{\Delta}{\mathalpha}{letters}{"01}
\DeclareMathSymbol{\Theta}{\mathalpha}{letters}{"02}
\DeclareMathSymbol{\Lambda}{\mathalpha}{letters}{"03}
\DeclareMathSymbol{\Xi}{\mathalpha}{letters}{"04}
\DeclareMathSymbol{\Pi}{\mathalpha}{letters}{"05}
\DeclareMathSymbol{\Sigma}{\mathalpha}{letters}{"06}
\DeclareMathSymbol{\Upsilon}{\mathalpha}{letters}{"07}
\DeclareMathSymbol{\Phi}{\mathalpha}{letters}{"08}
\DeclareMathSymbol{\Psi}{\mathalpha}{letters}{"09}
\DeclareMathSymbol{\Omega}{\mathalpha}{letters}{"0A}

\let\footnotesize\small

\if@custvec
\def\vec#1{\mathchoice{\mbox{\boldmath$\displaystyle#1$}}
{\mbox{\boldmath$\textstyle#1$}}
{\mbox{\boldmath$\scriptstyle#1$}}
{\mbox{\boldmath$\scriptscriptstyle#1$}}}
\fi

\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}
\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}
\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}
\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.8pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.3pt}<\cr}}}}}
\def\bbbr{{\rm I\!R}} %reelle Zahlen
\def\bbbm{{\rm I\!M}}
\def\bbbn{{\rm I\!N}} %natuerliche Zahlen
\def\bbbf{{\rm I\!F}}
\def\bbbh{{\rm I\!H}}
\def\bbbk{{\rm I\!K}}
\def\bbbp{{\rm I\!P}}
\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}
\def\bbbc{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm C$}\hbox{\hbox
to0pt{\kern0.4\wd0\vrule height0.9\ht0\hss}\box0}}}}
\def\bbbq{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.8\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.7\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm Q$}\hbox{\raise
0.15\ht0\hbox to0pt{\kern0.4\wd0\vrule height0.7\ht0\hss}\box0}}}}
\def\bbbt{{\mathchoice {\setbox0=\hbox{$\displaystyle\rm
T$}\hbox{\hbox to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle\rm T$}\hbox{\hbox
to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm T$}\hbox{\hbox
to0pt{\kern0.3\wd0\vrule height0.9\ht0\hss}\box0}}}}
\def\bbbs{{\mathchoice
{\setbox0=\hbox{$\displaystyle     \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.35\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.55\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\textstyle        \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.35\wd0\vrule height0.45\ht0\hss}\hbox
to0pt{\kern0.55\wd0\vrule height0.5\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptstyle      \rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.35\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.5\wd0\vrule height0.45\ht0\hss}\box0}}
{\setbox0=\hbox{$\scriptscriptstyle\rm S$}\hbox{\raise0.5\ht0\hbox
to0pt{\kern0.4\wd0\vrule height0.45\ht0\hss}\raise0.05\ht0\hbox
to0pt{\kern0.55\wd0\vrule height0.45\ht0\hss}\box0}}}}
\def\bbbz{{\mathchoice {\hbox{$\mathsf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\mathsf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\mathsf\scriptstyle Z\kern-0.3em Z$}}
{\hbox{$\mathsf\scriptscriptstyle Z\kern-0.2em Z$}}}}

\let\ts\,

\setlength\leftmargini  {17\p@}
\setlength\leftmargin    {\leftmargini}
\setlength\leftmarginii  {\leftmargini}
\setlength\leftmarginiii {\leftmargini}
\setlength\leftmarginiv  {\leftmargini}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}

\def\@listI{\leftmargin\leftmargini
            \parsep 0\p@ \@plus1\p@ \@minus\p@
            \topsep 8\p@ \@plus2\p@ \@minus4\p@
            \itemsep0\p@}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
              \labelwidth\leftmarginii
              \advance\labelwidth-\labelsep
              \topsep    0\p@ \@plus2\p@ \@minus\p@}
\def\@listiii{\leftmargin\leftmarginiii
              \labelwidth\leftmarginiii
              \advance\labelwidth-\labelsep
              \topsep    0\p@ \@plus\p@\@minus\p@
              \parsep    \z@
              \partopsep \p@ \@plus\z@ \@minus\p@}

\renewcommand\labelitemi{\normalfont\bfseries --}
\renewcommand\labelitemii{$\m@th\bullet$}

\setlength\arraycolsep{1.4\p@}
\setlength\tabcolsep{1.4\p@}

\def\tableofcontents{\chapter*{\contentsname\@mkboth{{\contentsname}}%
                                                    {{\contentsname}}}
 \def\authcount##1{\setcounter{auco}{##1}\setcounter{@auth}{1}}
 \def\lastand{\ifnum\value{auco}=2\relax
                 \unskip{} \andname\
              \else
                 \unskip \lastandname\
              \fi}%
 \def\and{\stepcounter{@auth}\relax
          \ifnum\value{@auth}=\value{auco}%
             \lastand
          \else
             \unskip,
          \fi}%
 \@starttoc{toc}\if@restonecol\twocolumn\fi}

\def\l@part#1#2{\addpenalty{\@secpenalty}%
   \addvspace{2em plus\p@}%  % space above part line
   \begingroup
     \parindent \z@
     \rightskip \z@ plus 5em
     \hrule\vskip5pt
     \large               % same size as for a contribution heading
     \bfseries\boldmath   % set line in boldface
     \leavevmode          % TeX command to enter horizontal mode.
     #1\par
     \vskip5pt
     \hrule
     \vskip1pt
     \nobreak             % Never break after part entry
   \endgroup}

\def\@dotsep{2}

\let\phantomsection=\relax

\def\hyperhrefextend{\ifx\hyper@anchor\@undefined\else
{}\fi}

\def\addnumcontentsmark#1#2#3{%
\addtocontents{#1}{\protect\contentsline{#2}{\protect\numberline
                     {\thechapter}#3}{\thepage}\hyperhrefextend}}%
\def\addcontentsmark#1#2#3{%
\addtocontents{#1}{\protect\contentsline{#2}{#3}{\thepage}\hyperhrefextend}}%
\def\addcontentsmarkwop#1#2#3{%
\addtocontents{#1}{\protect\contentsline{#2}{#3}{0}\hyperhrefextend}}%

\def\@adcmk[#1]{\ifcase #1 \or
\def\@gtempa{\addnumcontentsmark}%
  \or    \def\@gtempa{\addcontentsmark}%
  \or    \def\@gtempa{\addcontentsmarkwop}%
  \fi\@gtempa{toc}{chapter}%
}
\def\addtocmark{%
\phantomsection
\@ifnextchar[{\@adcmk}{\@adcmk[3]}%
}

\def\l@chapter#1#2{\addpenalty{-\@highpenalty}
 \vskip 1.0em plus 1pt \@tempdima 1.5em \begingroup
 \parindent \z@ \rightskip \@tocrmarg
 \advance\rightskip by 0pt plus 2cm
 \parfillskip -\rightskip \pretolerance=10000
 \leavevmode \advance\leftskip\@tempdima \hskip -\leftskip
 {\large\bfseries\boldmath#1}\ifx0#2\hfil\null
 \else
      \nobreak
      \leaders\hbox{$\m@th \mkern \@dotsep mu.\mkern
      \@dotsep mu$}\hfill
      \nobreak\hbox to\@pnumwidth{\hss #2}%
 \fi\par
 \penalty\@highpenalty \endgroup}

\def\l@title#1#2{\addpenalty{-\@highpenalty}
 \addvspace{8pt plus 1pt}
 \@tempdima \z@
 \begingroup
 \parindent \z@ \rightskip \@tocrmarg
 \advance\rightskip by 0pt plus 2cm
 \parfillskip -\rightskip \pretolerance=10000
 \leavevmode \advance\leftskip\@tempdima \hskip -\leftskip
 #1\nobreak
 \leaders\hbox{$\m@th \mkern \@dotsep mu.\mkern
 \@dotsep mu$}\hfill
 \nobreak\hbox to\@pnumwidth{\hss #2}\par
 \penalty\@highpenalty \endgroup}

\def\l@author#1#2{\addpenalty{\@highpenalty}
 \@tempdima=15\p@ %\z@
 \begingroup
 \parindent \z@ \rightskip \@tocrmarg
 \advance\rightskip by 0pt plus 2cm
 \pretolerance=10000
 \leavevmode \advance\leftskip\@tempdima %\hskip -\leftskip
 \textit{#1}\par
 \penalty\@highpenalty \endgroup}

\setcounter{tocdepth}{0}
\newdimen\tocchpnum
\newdimen\tocsecnum
\newdimen\tocsectotal
\newdimen\tocsubsecnum
\newdimen\tocsubsectotal
\newdimen\tocsubsubsecnum
\newdimen\tocsubsubsectotal
\newdimen\tocparanum
\newdimen\tocparatotal
\newdimen\tocsubparanum
\tocchpnum=\z@            % no chapter numbers
\tocsecnum=15\p@          % section 88. plus 2.222pt
\tocsubsecnum=23\p@       % subsection 88.8 plus 2.222pt
\tocsubsubsecnum=27\p@    % subsubsection 88.8.8 plus 1.444pt
\tocparanum=35\p@         % paragraph 88.8.8.8 plus 1.666pt
\tocsubparanum=43\p@      % subparagraph 88.8.8.8.8 plus 1.888pt
\def\calctocindent{%
\tocsectotal=\tocchpnum
\advance\tocsectotal by\tocsecnum
\tocsubsectotal=\tocsectotal
\advance\tocsubsectotal by\tocsubsecnum
\tocsubsubsectotal=\tocsubsectotal
\advance\tocsubsubsectotal by\tocsubsubsecnum
\tocparatotal=\tocsubsubsectotal
\advance\tocparatotal by\tocparanum}
\calctocindent

\def\l@section{\@dottedtocline{1}{\tocchpnum}{\tocsecnum}}
\def\l@subsection{\@dottedtocline{2}{\tocsectotal}{\tocsubsecnum}}
\def\l@subsubsection{\@dottedtocline{3}{\tocsubsectotal}{\tocsubsubsecnum}}
\def\l@paragraph{\@dottedtocline{4}{\tocsubsubsectotal}{\tocparanum}}
\def\l@subparagraph{\@dottedtocline{5}{\tocparatotal}{\tocsubparanum}}

\def\listoffigures{\@restonecolfalse\if@twocolumn\@restonecoltrue\onecolumn
 \fi\section*{\listfigurename\@mkboth{{\listfigurename}}{{\listfigurename}}}
 \@starttoc{lof}\if@restonecol\twocolumn\fi}
\def\l@figure{\@dottedtocline{1}{0em}{1.5em}}

\def\listoftables{\@restonecolfalse\if@twocolumn\@restonecoltrue\onecolumn
 \fi\section*{\listtablename\@mkboth{{\listtablename}}{{\listtablename}}}
 \@starttoc{lot}\if@restonecol\twocolumn\fi}
\let\l@table\l@figure

\renewcommand\listoffigures{%
    \section*{\listfigurename
      \@mkboth{\listfigurename}{\listfigurename}}%
    \@starttoc{lof}%
    }

\renewcommand\listoftables{%
    \section*{\listtablename
      \@mkboth{\listtablename}{\listtablename}}%
    \@starttoc{lot}%
    }

\ifx\oribibl\undefined
\ifx\citeauthoryear\undefined
\renewenvironment{thebibliography}[1]
     {\section*{\refname}
      \def\@biblabel##1{##1.}
      \small
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \if@openbib
              \advance\leftmargin\bibindent
              \itemindent -\bibindent
              \listparindent \itemindent
              \parsep \z@
            \fi
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \if@openbib
        \renewcommand\newblock{\par}%
      \else
        \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
      \fi
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.=\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}
\def\@lbibitem[#1]#2{\item[{[#1]}\hfill]\if@filesw
     {\let\protect\noexpand\immediate
     \write\@auxout{\string\bibcite{#2}{#1}}}\fi\ignorespaces}
\newcount\@tempcntc
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@ifundefined
       {b@\@citeb}{\@citeo\@tempcntb\m@ne\@citea\def\@citea{,}{\bfseries
        ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
    {\setbox\z@\hbox{\global\@tempcntc0\csname b@\@citeb\endcsname\relax}%
     \ifnum\@tempcntc=\z@ \@citeo\@tempcntb\m@ne
       \@citea\def\@citea{,}\hbox{\csname b@\@citeb\endcsname}%
     \else
      \advance\@tempcntb\@ne
      \ifnum\@tempcntb=\@tempcntc
      \else\advance\@tempcntb\m@ne\@citeo
      \@tempcnta\@tempcntc\@tempcntb\@tempcntc\fi\fi}}\@citeo}{#1}}
\def\@citeo{\ifnum\@tempcnta>\@tempcntb\else
               \@citea\def\@citea{,\,\hskip\z@skip}%
               \ifnum\@tempcnta=\@tempcntb\the\@tempcnta\else
               {\advance\@tempcnta\@ne\ifnum\@tempcnta=\@tempcntb \else
                \def\@citea{--}\fi
      \advance\@tempcnta\m@ne\the\@tempcnta\@citea\the\@tempcntb}\fi\fi}
\else
\renewenvironment{thebibliography}[1]
     {\section*{\refname}
      \small
      \list{}%
           {\settowidth\labelwidth{}%
            \leftmargin\parindent
            \itemindent=-\parindent
            \labelsep=\z@
            \if@openbib
              \advance\leftmargin\bibindent
              \itemindent -\bibindent
              \listparindent \itemindent
              \parsep \z@
            \fi
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{}}%
      \if@openbib
        \renewcommand\newblock{\par}%
      \else
        \renewcommand\newblock{\hskip .11em \@plus.33em \@minus.07em}%
      \fi
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.=\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}
      \def\@cite#1{#1}%
      \def\@lbibitem[#1]#2{\item[]\if@filesw
        {\def\protect##1{\string ##1\space}\immediate
      \write\@auxout{\string\bibcite{#2}{#1}}}\fi\ignorespaces}
   \fi
\else
\@cons\@openbib@code{\noexpand\small}
\fi

\def\idxquad{\hskip 10\p@}% space that divides entry from number

\def\@idxitem{\par\hangindent 10\p@}

\def\subitem{\par\setbox0=\hbox{--\enspace}% second order
                \noindent\hangindent\wd0\box0}% index entry

\def\subsubitem{\par\setbox0=\hbox{--\,--\enspace}% third
                \noindent\hangindent\wd0\box0}% order index entry

\def\indexspace{\par \vskip 10\p@ plus5\p@ minus3\p@\relax}

\renewenvironment{theindex}
               {\@mkboth{\indexname}{\indexname}%
                \thispagestyle{empty}\parindent\z@
                \parskip\z@ \@plus .3\p@\relax
                \let\item\par
                \def\,{\relax\ifmmode\mskip\thinmuskip
                             \else\hskip0.2em\ignorespaces\fi}%
                \normalfont\small
                \begin{multicols}{2}[\@makeschapterhead{\indexname}]%
                }
                {\end{multicols}}

\renewcommand\footnoterule{%
  \kern-3\p@
  \hrule\@width 2truecm
  \kern2.6\p@}
  \newdimen\fnindent
  \fnindent1em
\long\def\@makefntext#1{%
    \parindent \fnindent%
    \leftskip \fnindent%
    \noindent
    \llap{\hb@xt@1em{\hss\@makefnmark\ }}\ignorespaces#1}

\long\def\@makecaption#1#2{%
  \small
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\bfseries #1.} #2}%
  \ifdim \wd\@tempboxa >\hsize
    {\bfseries #1.} #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}

\def\fps@figure{htbp}
\def\fnum@figure{\figurename\thinspace\thefigure}
\def \@floatboxreset {%
        \reset@font
        \small
        \@setnobreak
        \@setminipage
}
\def\fps@table{htbp}
\def\fnum@table{\tablename~\thetable}
\renewenvironment{table}
               {\setlength\abovecaptionskip{0\p@}%
                \setlength\belowcaptionskip{10\p@}%
                \@float{table}}
               {\end@float}
\renewenvironment{table*}
               {\setlength\abovecaptionskip{0\p@}%
                \setlength\belowcaptionskip{10\p@}%
                \@dblfloat{table}}
               {\end@dblfloat}

\long\def\@caption#1[#2]#3{\par\addcontentsline{\csname
  ext@#1\endcsname}{#1}{\protect\numberline{\csname
  the#1\endcsname}{\ignorespaces #2}}\begingroup
    \@parboxrestore
    \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}

% LaTeX does not provide a command to enter the authors institute
% addresses. The \institute command is defined here.

\newcounter{@inst}
\newcounter{@auth}
\newcounter{auco}
\newdimen\instindent
\newbox\authrun
\newtoks\authorrunning
\newtoks\tocauthor
\newbox\titrun
\newtoks\titlerunning
\newtoks\toctitle

\def\clearheadinfo{\gdef\@author{No Author Given}%
                   \gdef\@title{No Title Given}%
                   \gdef\@subtitle{}%
                   \gdef\@institute{No Institute Given}%
                   \gdef\@thanks{}%
                   \global\titlerunning={}\global\authorrunning={}%
                   \global\toctitle={}\global\tocauthor={}}

\def\institute#1{\gdef\@institute{#1}}

\def\institutename{\par
 \begingroup
 \parskip=\z@
 \parindent=\z@
 \setcounter{@inst}{1}%
 \def\and{\par\stepcounter{@inst}%
 \noindent$^{\the@inst}$\enspace\ignorespaces}%
 \setbox0=\vbox{\def\thanks##1{}\@institute}%
 \ifnum\c@@inst=1\relax
   \gdef\fnnstart{0}%
 \else
   \xdef\fnnstart{\c@@inst}%
   \setcounter{@inst}{1}%
   \noindent$^{\the@inst}$\enspace
 \fi
 \ignorespaces
 \@institute\par
 \endgroup}

\def\@fnsymbol#1{\ensuremath{\ifcase#1\or\star\or{\star\star}\or
   {\star\star\star}\or \dagger\or \ddagger\or
   \mathchar "278\or \mathchar "27B\or \|\or **\or \dagger\dagger
   \or \ddagger\ddagger \else\@ctrerr\fi}}

\def\inst#1{\unskip$^{#1}$}
\def\orcidID#1{\unskip$^{[#1]}$} % added MR 2018-03-10
\def\fnmsep{\unskip$^,$}
\def\email#1{{\tt#1}}

\AtBeginDocument{\@ifundefined{url}{\def\url#1{#1}}{}%
\@ifpackageloaded{babel}{%
\@ifundefined{extrasenglish}{}{\addto\extrasenglish{\switcht@albion}}%
\@ifundefined{extrasfrenchb}{}{\addto\extrasfrenchb{\switcht@francais}}%
\@ifundefined{extrasgerman}{}{\addto\extrasgerman{\switcht@deutsch}}%
\@ifundefined{extrasngerman}{}{\addto\extrasngerman{\switcht@deutsch}}%
}{\switcht@@therlang}%
\providecommand{\keywords}[1]{\def\and{{\textperiodcentered} }%
\par\addvspace\baselineskip
\noindent\keywordname\enspace\ignorespaces#1}%
\@ifpackageloaded{hyperref}{%
\def\doi#1{\href{https://doi.org/#1}{https://doi.org/#1}}}{
\def\doi#1{https://doi.org/#1}}
}
\def\homedir{\~{ }}

\def\subtitle#1{\gdef\@subtitle{#1}}
\clearheadinfo
%
%%% to avoid hyperref warnings
\providecommand*{\toclevel@author}{999}
%%% to make title-entry parent of section-entries
\providecommand*{\toclevel@title}{0}
%
\renewcommand\maketitle{\newpage
\phantomsection
  \refstepcounter{chapter}%
  \stepcounter{section}%
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{figure}{0}
  \setcounter{table}{0}
  \setcounter{equation}{0}
  \setcounter{footnote}{0}%
  \begingroup
    \parindent=\z@
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \if@twocolumn
      \ifnum \col@number=\@ne
        \@maketitle
      \else
        \twocolumn[\@maketitle]%
      \fi
    \else
      \newpage
      \global\@topnum\z@   % Prevents figures from going at top of page.
      \@maketitle
    \fi
    \thispagestyle{empty}\@thanks
%
    \def\\{\unskip\ \ignorespaces}\def\inst##1{\unskip{}}%
    \def\thanks##1{\unskip{}}\def\fnmsep{\unskip}%
    \instindent=\hsize
    \advance\instindent by-\headlineindent
    \if!\the\toctitle!\addcontentsline{toc}{title}{\@title}\else
       \addcontentsline{toc}{title}{\the\toctitle}\fi
    \if@runhead
       \if!\the\titlerunning!\else
         \edef\@title{\the\titlerunning}%
       \fi
       \global\setbox\titrun=\hbox{\small\rm\unboldmath\ignorespaces\@title}%
       \ifdim\wd\titrun>\instindent
          \typeout{Title too long for running head. Please supply}%
          \typeout{a shorter form with \string\titlerunning\space prior to
                   \string\maketitle}%
          \global\setbox\titrun=\hbox{\small\rm
          Title Suppressed Due to Excessive Length}%
       \fi
       \xdef\@title{\copy\titrun}%
    \fi
%
    \if!\the\tocauthor!\relax
      {\def\and{\noexpand\protect\noexpand\and}%
       \def\inst##1{}%    added MR 2017-09-20 to remove inst numbers from the TOC
       \def\orcidID##1{}% added MR 2017-09-20 to remove ORCID ids from the TOC
      \protected@xdef\toc@uthor{\@author}}%
    \else
      \def\\{\noexpand\protect\noexpand\newline}%
      \protected@xdef\scratch{\the\tocauthor}%
      \protected@xdef\toc@uthor{\scratch}%
    \fi
    \addtocontents{toc}{\noexpand\protect\noexpand\authcount{\the\c@auco}}%
    \addcontentsline{toc}{author}{\toc@uthor}%
    \if@runhead
       \if!\the\authorrunning!
         \value{@inst}=\value{@auth}%
         \setcounter{@auth}{1}%
       \else
         \edef\@author{\the\authorrunning}%
       \fi
       \global\setbox\authrun=\hbox{\def\inst##1{}%    added MR 2017-09-20 to remove inst numbers from the runninghead
                                    \def\orcidID##1{}% added MR 2017-09-20 to remove ORCID ids from the runninghead
                                    \small\unboldmath\@author\unskip}%
       \ifdim\wd\authrun>\instindent
          \typeout{Names of authors too long for running head. Please supply}%
          \typeout{a shorter form with \string\authorrunning\space prior to
                   \string\maketitle}%
          \global\setbox\authrun=\hbox{\small\rm
          Authors Suppressed Due to Excessive Length}%
       \fi
       \xdef\@author{\copy\authrun}%
       \markboth{\@author}{\@title}%
     \fi
  \endgroup
  \setcounter{footnote}{\fnnstart}%
  \clearheadinfo}
%
\def\@maketitle{\newpage
 \markboth{}{}%
 \def\lastand{\ifnum\value{@inst}=2\relax
                 \unskip{} \andname\
              \else
                 \unskip \lastandname\
              \fi}%
 \def\and{\stepcounter{@auth}\relax
          \ifnum\value{@auth}=\value{@inst}%
             \lastand
          \else
             \unskip,
          \fi}%
 \begin{center}%
 \let\newline\\
 {\Large \bfseries\boldmath
  \pretolerance=10000
  \@title \par}\vskip .8cm
\if!\@subtitle!\else {\large \bfseries\boldmath
  \vskip -.65cm
  \pretolerance=10000
  \@subtitle \par}\vskip .8cm\fi
 \setbox0=\vbox{\setcounter{@auth}{1}\def\and{\stepcounter{@auth}}%
 \def\thanks##1{}\@author}%
 \global\value{@inst}=\value{@auth}%
 \global\value{auco}=\value{@auth}%
 \setcounter{@auth}{1}%
{\lineskip .5em
\noindent\ignorespaces
\@author\vskip.35cm}
 {\small\institutename}
 \end{center}%
 }

% definition of the "\spnewtheorem" command.
%
% Usage:
%
%     \spnewtheorem{env_nam}{caption}[within]{cap_font}{body_font}
% or  \spnewtheorem{env_nam}[numbered_like]{caption}{cap_font}{body_font}
% or  \spnewtheorem*{env_nam}{caption}{cap_font}{body_font}
%
% New is "cap_font" and "body_font". It stands for
% fontdefinition of the caption and the text itself.
%
% "\spnewtheorem*" gives a theorem without number.
%
% A defined spnewthoerem environment is used as described
% by Lamport.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@thmcountersep{}
\def\@thmcounterend{.}

\def\spnewtheorem{\@ifstar{\@sthm}{\@Sthm}}

% definition of \spnewtheorem with number

\def\@spnthm#1#2{%
  \@ifnextchar[{\@spxnthm{#1}{#2}}{\@spynthm{#1}{#2}}}
\def\@Sthm#1{\@ifnextchar[{\@spothm{#1}}{\@spnthm{#1}}}

\def\@spxnthm#1#2[#3]#4#5{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}\@addtoreset{#1}{#3}%
   \expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
     \csname the#3\endcsname \noexpand\@thmcountersep \@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
                              \global\@namedef{end#1}{\@endtheorem}}}

\def\@spynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\@definecounter{#1}%
   \expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
   \expandafter\xdef\csname #1name\endcsname{#2}%
   \global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#3}{#4}}%
                               \global\@namedef{end#1}{\@endtheorem}}}

\def\@spothm#1[#2]#3#4#5{%
  \@ifundefined{c@#2}{\@latexerr{No theorem environment `#2' defined}\@eha}%
  {\expandafter\@ifdefinable\csname #1\endcsname
  {\newaliascnt{#1}{#2}%
  \expandafter\xdef\csname #1name\endcsname{#3}%
  \global\@namedef{#1}{\@spthm{#1}{\csname #1name\endcsname}{#4}{#5}}%
  \global\@namedef{end#1}{\@endtheorem}}}}

\def\@spthm#1#2#3#4{\topsep 7\p@ \@plus2\p@ \@minus4\p@
\refstepcounter{#1}%
\@ifnextchar[{\@spythm{#1}{#2}{#3}{#4}}{\@spxthm{#1}{#2}{#3}{#4}}}

\def\@spxthm#1#2#3#4{\@spbegintheorem{#2}{\csname the#1\endcsname}{#3}{#4}%
                    \ignorespaces}

\def\@spythm#1#2#3#4[#5]{\@spopargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}

\def\@spbegintheorem#1#2#3#4{\trivlist
                 \item[\hskip\labelsep{#3#1\ #2\@thmcounterend}]#4}

\def\@spopargbegintheorem#1#2#3#4#5{\trivlist
      \item[\hskip\labelsep{#4#1\ #2}]{#4(#3)\@thmcounterend\ }#5}

% definition of \spnewtheorem* without number

\def\@sthm#1#2{\@Ynthm{#1}{#2}}

\def\@Ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
   {\global\@namedef{#1}{\@Thm{\csname #1name\endcsname}{#3}{#4}}%
    \expandafter\xdef\csname #1name\endcsname{#2}%
    \global\@namedef{end#1}{\@endtheorem}}}

\def\@Thm#1#2#3{\topsep 7\p@ \@plus2\p@ \@minus4\p@
\@ifnextchar[{\@Ythm{#1}{#2}{#3}}{\@Xthm{#1}{#2}{#3}}}

\def\@Xthm#1#2#3{\@Begintheorem{#1}{#2}{#3}\ignorespaces}

\def\@Ythm#1#2#3[#4]{\@Opargbegintheorem{#1}
       {#4}{#2}{#3}\ignorespaces}

\def\@Begintheorem#1#2#3{#3\trivlist
                           \item[\hskip\labelsep{#2#1\@thmcounterend}]}

\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
      \item[\hskip\labelsep{#3#1}]{#3(#2)\@thmcounterend\ }}

\if@envcntsect
   \def\@thmcountersep{.}
   \spnewtheorem{theorem}{Theorem}[section]{\bfseries}{\itshape}
\else
   \spnewtheorem{theorem}{Theorem}{\bfseries}{\itshape}
   \if@envcntreset
      \@addtoreset{theorem}{section}
   \else
      \@addtoreset{theorem}{chapter}
   \fi
\fi

%definition of divers theorem environments
\spnewtheorem*{claim}{Claim}{\itshape}{\rmfamily}
\spnewtheorem*{proof}{Proof}{\itshape}{\rmfamily}
\if@envcntsame % alle Umgebungen wie Theorem.
   \def\spn@wtheorem#1#2#3#4{\@spothm{#1}[theorem]{#2}{#3}{#4}}
\else % alle Umgebungen mit eigenem Zaehler
   \if@envcntsect % mit section numeriert
      \def\spn@wtheorem#1#2#3#4{\@spxnthm{#1}{#2}[section]{#3}{#4}}
   \else % nicht mit section numeriert
      \if@envcntreset
         \def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
                                   \@addtoreset{#1}{section}}
      \else
         \def\spn@wtheorem#1#2#3#4{\@spynthm{#1}{#2}{#3}{#4}
                                   \@addtoreset{#1}{chapter}}%
      \fi
   \fi
\fi
\spn@wtheorem{case}{Case}{\itshape}{\rmfamily}
\spn@wtheorem{conjecture}{Conjecture}{\itshape}{\rmfamily}
\spn@wtheorem{corollary}{Corollary}{\bfseries}{\itshape}
\spn@wtheorem{definition}{Definition}{\bfseries}{\itshape}
\spn@wtheorem{example}{Example}{\itshape}{\rmfamily}
\spn@wtheorem{exercise}{Exercise}{\itshape}{\rmfamily}
\spn@wtheorem{lemma}{Lemma}{\bfseries}{\itshape}
\spn@wtheorem{note}{Note}{\itshape}{\rmfamily}
\spn@wtheorem{problem}{Problem}{\itshape}{\rmfamily}
\spn@wtheorem{property}{Property}{\itshape}{\rmfamily}
\spn@wtheorem{proposition}{Proposition}{\bfseries}{\itshape}
\spn@wtheorem{question}{Question}{\itshape}{\rmfamily}
\spn@wtheorem{solution}{Solution}{\itshape}{\rmfamily}
\spn@wtheorem{remark}{Remark}{\itshape}{\rmfamily}

\def\@takefromreset#1#2{%
    \def\@tempa{#1}%
    \let\@tempd\@elt
    \def\@elt##1{%
        \def\@tempb{##1}%
        \ifx\@tempa\@tempb\else
            \@addtoreset{##1}{#2}%
        \fi}%
    \expandafter\expandafter\let\expandafter\@tempc\csname cl@#2\endcsname
    \expandafter\def\csname cl@#2\endcsname{}%
    \@tempc
    \let\@elt\@tempd}

\def\theopargself{\def\@spopargbegintheorem##1##2##3##4##5{\trivlist
      \item[\hskip\labelsep{##4##1\ ##2}]{##4##3\@thmcounterend\ }##5}
                  \def\@Opargbegintheorem##1##2##3##4{##4\trivlist
      \item[\hskip\labelsep{##3##1}]{##3##2\@thmcounterend\ }}
      }

\renewenvironment{abstract}{%
      \list{}{\advance\topsep by0.35cm\relax\small
      \leftmargin=1cm
      \labelwidth=\z@
      \listparindent=\z@
      \itemindent\listparindent
      \rightmargin\leftmargin}\item[\hskip\labelsep
                                    \bfseries\abstractname]}
    {\endlist}

\newdimen\headlineindent             % dimension for space between
\headlineindent=1.166cm              % number and text of headings.

\def\ps@headings{\let\@mkboth\@gobbletwo
   \let\@oddfoot\@empty\let\@evenfoot\@empty
   \def\@evenhead{\normalfont\small\rlap{\thepage}\hspace{\headlineindent}%
                  \leftmark\hfil}
   \def\@oddhead{\normalfont\small\hfil\rightmark\hspace{\headlineindent}%
                 \llap{\thepage}}
   \def\chaptermark##1{}%
   \def\sectionmark##1{}%
   \def\subsectionmark##1{}}

\def\ps@titlepage{\let\@mkboth\@gobbletwo
   \let\@oddfoot\@empty\let\@evenfoot\@empty
   \def\@evenhead{\normalfont\small\rlap{\thepage}\hspace{\headlineindent}%
                  \hfil}
   \def\@oddhead{\normalfont\small\hfil\hspace{\headlineindent}%
                 \llap{\thepage}}
   \def\chaptermark##1{}%
   \def\sectionmark##1{}%
   \def\subsectionmark##1{}}

\if@runhead\ps@headings\else
\ps@empty\fi

\setlength\arraycolsep{1.4\p@}
\setlength\tabcolsep{1.4\p@}

\endinput
%end of file llncs.cls


==> problem.tex <==
\section{Definitions and Problem Statement}
\anis{these definitions can be written in more compact form to save space. It is fine if we remove the definition box and simply write them in text. Since they are very well-known problems and also we defined them earlier too (in fact, check if can remove them). Only keep the Problem definition as it is.}
\begin{definition}[Dominating Set]
Let $G(V,E)$ be a graph with vertex(node) set $V$ and edge set $E$. We call a subset $D\subset V$, a dominating set for the graph $G$ if for any $v\in V$, either $v\in D$ there exists a node $u\in D$ such that $u$ is a neighbour of $v$.
\end{definition}
A trivial dominating set for any graph $G$ happens to be the whole node set $V$. Therefore, quite naturally, we want to find dominating sets that have a low cardinality. In this context, we define another useful term, the 'minimal dominating set'. 


\begin{definition}[Minimal Dominating Set]
A set of nodes, $D\subset V$ with the following properties is called a minimal dominating set:
\begin{enumerate}
    \item $D$ is a dominating set
    \item no proper subset of $D$ is a dominating set of $G$
\end{enumerate}
\end{definition}
We now define another term, the 'minimum dominating set', which represents an optimal dominating set in terms of the set size. 

\begin{definition}[Minimum Dominating Set]
A set of nodes, $D\subset V$ with the following properties is called a minimum dominating set:
\begin{enumerate}
    \item $D$ is a dominating set
    \item for any dominating set $D'$ of $G$, $|D|\leq |D'|$
\end{enumerate}
where $|\cdot|$ represents the size of a set.
\end{definition}

% In this paper, we also take up the well-studied problem of finding a connected dominating set. 
% \begin{definition}[Connected Dominating Set]
%  We call a subset $D\subset V$, a connected dominating set if it satisfies the following properties. 
% \begin{enumerate}
%     \item $D$ is a dominating set.
%     \item $D$ induces a connected sub-graph of $G$.
% \end{enumerate}
% \end{definition}
% For any connected graph, $G(V,E)$, $V$ itself gives us a trivial connected dominating set. Therefore, we shall focus on minimising the size of the connected dominating set. 

With all the definitions and model descriptions in place, we formally state our problem.  

\begin{definition}[Problem Definition]
Consider an undirected, simple connected $n$-node graph $G(V,E)$, with $n$ mobile robots placed on the nodes of $G$. The mobile robots can start at two possible opening configurations - the rooted configuration or the arbitrary configuration. We want to use mobile robots to design algorithms that solve the following problems:
\begin{enumerate}
    \item \textbf{The Minimal Dominating Set Problem} - The robots irrespective of how they are initially placed, rearrange and colour themselves in such a way that a minimal dominating set for $G$ is identified.
    \item \textbf{The Optimal Dominating Set Approximation} - The robots irrespective of how they are initially placed, rearrange and colour themselves in such a way that a dominating set for $G$ of size at most $\mathbf{r}$ times of the minimum dominating set is identified. Here $\mathbf{r}$ is the approximation ratio to the minimum dominating set.
    % \item \textbf{The Connected Dominating Set Problem} - The robots irrespective of how they are initially placed, rearrange and colour themselves in such a way that a connected dominating set for $G$ is identified.
    
\end{enumerate}

\end{definition}
% \begin{definition}[minimum $1$-hop covering]
% Consider an undirected, simple connected $n$-node graph $G=(V,E)$ with a node $v_s\in V$, which is an infinite source of mobile robots. The \textbf{minimum 1-hop covering problem} asks to disperse $|D^1|\leq n$ robots from $V_s$ into a set of nodes $D^1\subset V $ such that
% \begin{enumerate}
%     \item the dispersed robots form an \textit{1-hop covering} of $G$
%     \item The size of $D^1$ is minimum
% \end{enumerate}
% \end{definition}


% \begin{definition}[minimum $k$-hop covering]
% Consider an undirected, simple connected $n$-node graph $G=(V,E)$ with a node $v_s\in V$, which is an infinite source of mobile robots. The \textbf{minimum k-hop covering problem} asks to disperse $|D^k|\leq n$ robots from $V_s$ into set of nodes $D^k\subset V $ such that
% \begin{enumerate}
%     \item the dispersed robots form a \textit{k-hop covering} of $G$
%     \item The size of $D^k$ is minimum
% \end{enumerate}
% \end{definition}


% \begin{definition}[minimal $1$-hop covering]
% Consider an undirected, simple connected $n$-node graph $G=(V,E)$ with a node $v_s\in V$, which is an infinite source of mobile robots. The \textbf{minimal 1-hop covering problem} asks to disperse $|D^1|\leq n$ robots from $V_s$ into a set of nodes $D^1\subset V $ such that
% \begin{enumerate}
%     \item the dispersed robots form an \textit{1-hop covering} of $G$
%     \item there does not exist any configuration of robots, which, when placed on the nodes of $D\subsetneqq D^1$ solves the \textit{1-hop covering problem}
% \end{enumerate}
% \end{definition}


% \begin{definition}[minimal $k$-hop covering]
% Consider an undirected, simple connected $n$-node graph $G=(V,E)$ with a node $v_s\in V$, which is an infinite source of mobile robots. The \textbf{minimal k-hop covering problem} asks to disperse $|D^k|\leq n$ robots from $V_s$ into set of nodes $D^k\subset V $ such that
% \begin{enumerate}
%     \item the dispersed robots form a \textit{k-hop covering} of $G$
%     \item there does not exist any configuration of robots, which, when placed on the nodes of $D\subsetneqq D^1$ solves the \textit{k-hop covering problem}
% \end{enumerate}
% \end{definition}
\endinput
